A Residual Encoder-Decoder Network for Segmentation of Retinal Image-Based Exudates in Diabetic Retinopathy Screening

Diabetic retinopathy refers to the pathology of the retina induced by diabetes and is one of the leading causes of preventable blindness in the world. Early detection of diabetic retinopathy is critical to avoid vision problem through continuous screening and treatment. In traditional clinical practice, the involved lesions are manually detected using photographs of the fundus. However, this task is cumbersome and time-consuming and requires intense effort due to the small size of lesion and low contrast of the images. Thus, computer-assisted diagnosis of diabetic retinopathy based on the detection of red lesions is actively being explored recently. In this paper, we present a convolutional neural network with residual skip connection for the segmentation of exudates in retinal images. To improve the performance of network architecture, a suitable image augmentation technique is used. The proposed network can robustly segment exudates with high accuracy, which makes it suitable for diabetic retinopathy screening. Comparative performance analysis of three benchmark databases: HEI-MED, E-ophtha, and DiaretDB1 is presented. It is shown that the proposed method achieves accuracy (0.98, 0.99, 0.98) and sensitivity (0.97, 0.92, and 0.95) on E-ophtha, HEI-MED, and DiaReTDB1, respectively.

==> Tables/ClassifierComparion.tex <==
    \begin{tabular}{clllll}
    \toprule
          &       & \multicolumn{1}{p{6.645em}}{\textbf{Support vector machine}} & \multicolumn{1}{p{6.645em}}{\textbf{ Random forest }} & \multicolumn{1}{p{6.645em}}{\textbf{AdaBoostM1 }} & \multicolumn{1}{p{6.645em}}{\textbf{RusBoost}} \\
    \midrule
    \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{sideways}\textbf{DRIONS}\end{sideways}}} & \textcolor[rgb]{ .137,  .122,  .125}{AOL } & 0.809 & 0.821 & 0.786 & 0.835 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Dice} & 0.892 & 0.899 & 0.872 & 0.902 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Acc } & 0.992 & 0.993 & 0.992 & 0.993 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SN} & 0.969 & 0.948 & 0.845 & 0.959 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SP} & 0.993 & 0.994 & 0.997 & 0.993 \\
    \midrule
    \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{sideways}\textbf{MESSIDOR}\end{sideways}}} & \textcolor[rgb]{ .137,  .122,  .125}{AOL } & 0.733 & 0.747 & 0.742 & 0.743 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Dice} & 0.841 & 0.851 & 0.847 & 0.847 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Acc } & 0.988 & 0.988 & 0.988 & 0.988 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SN} & 0.934 & 0.953 & 0.888 & 0.912 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SP} & 0.987 & 0.988 & 0.953 & 0.988 \\
    \midrule
    \multicolumn{1}{c}{\multirow{5}[2]{*}{\begin{sideways}\textbf{ONHSD}\end{sideways}}} & \textcolor[rgb]{ .137,  .122,  .125}{AOL } & 0.783 & 0.824 & 0.797 & 0.826 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Dice} & 0.875 & 0.897 & 0.879 & 0.902 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{Acc } & 0.99  & 0.993 & 0.992 & 0.993 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SN} & 0.926 & 0.924 & 0.877 & 0.952 \\
          & \textcolor[rgb]{ .137,  .122,  .125}{SP} & 0.991 & 0.995 & 0.996 & 0.994 \\
    \bottomrule
    \end{tabular}%


==> Tables/Comparison.tex <==
   \begin{tabular}{rrp{19.07em}p{8.145em}r}
    \toprule
    \multicolumn{1}{c}{\textbf{No.}} & \multicolumn{1}{c}{\textbf{Author}} & \multicolumn{1}{c}{\textbf{Method+Brief Detail}} & \multicolumn{1}{c}{\textbf{Database}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\
    \midrule
          &       & Morphology based preprocessing  & DRIONS & 0.9986 \\
    \multicolumn{1}{c}{1} & \multicolumn{1}{p{7.645em}} {\cite{zahoor2017fast}} & followed by circular Hough transform for OD localization & MESSIDOR & 0.9918 \\
          & \multicolumn{1}{p{7.645em}}{} &  & DRIVE & 0.998 \\
\cmidrule{4-5}          &       & Structured learning based OD segmentation  & DRIONS & 0.976 \\
    \multicolumn{1}{c}{2} & \multicolumn{1}{p{7.645em}}{\cite{fan2018optic}} &  & MESSIDOR & 0.977 \\
          &       & \multicolumn{1}{r}{} & ONHSD & 0.9895 \\
\cmidrule{4-5}          &       & OD extraction by watershed segmentation  & DRIONS & 0.9689 \\
    \multicolumn{1}{c}{3} & \multicolumn{1}{p{7.645em}}{\cite{walter2002contribution}} &   & MESSIDOR & ----- \\
          &       &   & ONHSD &  ----- \\
\cmidrule{4-5}          &       & PCA and mathematical morphology   & DRIONS & 0.9934 \\
    \multicolumn{1}{c}{4} & \multicolumn{1}{p{7.645em}}{\cite{morales2013automatic}} &  based OD segmentation & MESSIDOR & 0.9949 \\
          &       &   & ONHSD & 0.9941 \\
\cmidrule{4-5}          &       & Morphology based OD localization   & DRIONS & 0.9909 \\
    \multicolumn{1}{c}{5} & \multicolumn{1}{l}{\cite{abdullah2016localization}} & segmentation based on grow-cut algorithm  & MESSIDOR & 0.9925 \\
          &       & & ONHSD & 1 \\
\cmidrule{4-5}    \multicolumn{1}{c}{6} &       & Multi-parametric optic disc Segmentation & DRIONS & 0.993 \\
          & \multicolumn{1}{l}{Proposed} &  using superpixel based feature  & MESSIDOR & 0.998 \\
          &       & classification & ONHSD & 0.997 \\
    \bottomrule
    \end{tabular}%


==> Tables/Comparison2.tex <==
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Performance measures$\rightarrow$} & \multicolumn{1}{c}{\textbf{Sensitivity}} & \multicolumn{1}{c}{\textbf{Specificity}} & \multicolumn{1}{c}{\textbf{AOL}} & \multicolumn{1}{c}{\textbf{Dice}} & \multicolumn{1}{c}{\textbf{Accuracy}} \\
    \midrule
    \textbf{Method$\downarrow$} &       &       &       &       &  \\
\cmidrule{1-1}    \textbf{DRIONS} &       &       &       &       &  \\
    \midrule
    \cite{zahoor2017fast} & 0.938 & 0.999 & 0.884 & 0.889 & 0.998 \\
    \cite{fan2018optic} & 0.8957 & ----- & 0.8473 & 0.9137 & 0.976 \\
    \cite{walter2002contribution} & 0.6715 & ----- & 0.6227 & 0.6813 & 0.9689 \\
    \cite{morales2013automatic} & 0.928 & ----- & 0.842 & 0.908 & 0.993 \\
    \cite{abdullah2016localization} & 0.8508 & 0.9966 & 0.851 & 0.9102 & 0.9549 \\
    Proposed & 0.969 & 0.994 & 0.821 & 0.899 & 0.993 \\
    \midrule
    \textbf{Messidor} &       &       &       &       &  \\
    \midrule
    \cite{zahoor2017fast} & 0.889 & 0.997 & 0.844 & 0.903 & 0.991 \\
    \cite{fan2018optic} & 0.9212 & ----- & 0.8636 & 0.9196 & 0.977 \\
    \cite{morales2013automatic} & 0.93  & ----- & 0.8228 & 0.895 & 0.9949 \\
    \cite{abdullah2016localization} & 0.8954 & 0.9995 & 0.879 & 0.9339 & 0.9989 \\
    Proposed & 0.948 & 0.988 & 0.747 & 0.851 & 0.988 \\
    \midrule
    \textbf{ONHSD} &       &       &       &       &  \\
    \midrule
    \cite{zahoor2017fast} & 0.9077 & ----- & 0.8346 & 0.9032 & 0.9895 \\
     \cite{morales2013automatic} & 0.931 & ----- & 0.8045 & 0.8867 & 0.9941 \\
    \cite{abdullah2016localization} & 0.8857 & 0.9992 & 0.861 & 0.9197 & 0.9967 \\
    Proposed & 0.924 & 0.995 & 0.824 & 0.897 & 0.993 \\
    \bottomrule
    \end{tabular}%


==> Tables/Features.tex <==
\begin{tabular}{p{10em}|c}
    \multicolumn{1}{p{10em}}{\textbf{Feature Name}} & \multicolumn{1}{p{9.07em}}{\textbf{Number of Features}} \bigstrut[b]\\
    \hline
    \textbf{Statistical based features } & 5 \bigstrut[t]\\
    \textbf{Texton histogram} & 6 \\
    \textbf{Fractal features} & 6 \\
    \textbf{Total} & 17 \\
    \hline
    \end{tabular}%


==> Tables/Superpixel.tex <==
\begin{tabular}{p{8.27em}cccccc}
    \hline
    \textbf{Size of Superpixel } & 4     & 6     & 8     & 10    & 15 \bigstrut\\
    \hline
    \textbf{Dice coefficient} & 0.94  & 0.92  & 0.89  & 0.88  & 0.81  \bigstrut\\
    \hline
    \end{tabular}% 

==> Tables/TimingComparison.tex <==

    \begin{tabular}{l|c|c|c}
    \hline
    \multicolumn{1}{c|}{\textbf{Time (seconds)}} &
      \textbf{Classifier Training } &
      \textbf{Feature Computation} &
      \textbf{Feature Selection + Classification}
      \bigstrut\\
    \hline
    \multicolumn{1}{r|}{Support Vector Machine} &
      36.3 &
      \multirow{4}[2]{*}{19.5} &
      \multirow{4}[2]{*}{2.5}
      \bigstrut[t]\\
    Random Forest &
      9.1 &
       &
      
      \\
    AdaBoostM1 &
      7.5 &
       &
      
      \\
    RusBoost &
      12.9 &
       &
      
      \bigstrut[b]\\
    \hline
    \end{tabular}%


==> Tables/comparisonDB.tex <==
    \begin{tabular}{cp{8.645em}ccc}
    \hline
    \multicolumn{1}{p{4.215em}}{\textcolor[rgb]{ .137,  .122,  .125}{\textbf{Sr. No}}} & \textcolor[rgb]{ .137,  .122,  .125}{\textbf{Method name}} & \multicolumn{1}{p{7.145em}}{\textcolor[rgb]{ .137,  .122,  .125}{\textbf{Sensitivity}}} & \multicolumn{1}{p{7em}}{\textcolor[rgb]{ .137,  .122,  .125}{\textbf{PPV }}} & \multicolumn{1}{p{6.5em}}{\textcolor[rgb]{ .137,  .122,  .125}{\textbf{F-score}}} \bigstrut\\
    \hline
    1     & Walter [11] & \textcolor[rgb]{ .137,  .122,  .125}{0.69} & \textcolor[rgb]{ .137,  .122,  .125}{0.48} & \textcolor[rgb]{ .137,  .122,  .125}{0.57} \bigstrut[t]\\
    2     & Sánchez [48]  & \textcolor[rgb]{ .137,  .122,  .125}{0.34} & \textcolor[rgb]{ .137,  .122,  .125}{0.61} & \textcolor[rgb]{ .137,  .122,  .125}{0.44} \\
    3     & Harangi [13] & \textcolor[rgb]{ .137,  .122,  .125}{0.66} & \textcolor[rgb]{ .137,  .122,  .125}{0.65} & \textcolor[rgb]{ .137,  .122,  .125}{0.66} \\
    4     & Amel [20]  & \textcolor[rgb]{ .137,  .122,  .125}{0.41} & \textcolor[rgb]{ .137,  .122,  .125}{0.09} & \textcolor[rgb]{ .137,  .122,  .125}{0.15} \\
    5     & Harangi [22]  & \textcolor[rgb]{ .137,  .122,  .125}{0.71} & \textcolor[rgb]{ .137,  .122,  .125}{0.66} & \textcolor[rgb]{ .137,  .122,  .125}{0.68} \\
    \textcolor[rgb]{ .137,  .122,  .125}{6} & \textcolor[rgb]{ .137,  .122,  .125}{Proposed} & \textcolor[rgb]{ .137,  .122,  .125}{0.78} & \textcolor[rgb]{ .137,  .122,  .125}{0.78} & \textcolor[rgb]{ .137,  .122,  .125}{0.78} \bigstrut[b]\\
    \hline
    \end{tabular}%

